WiFiTrace: Network-based Contact Tracing for Infectious Diseases Using Passive WiFi Sensing

Contact tracing is a well-established and effective approach for the containment of the spread of infectious diseases. While Bluetooth-based contact tracing method using phones has become popular recently, these approaches suffer from the need for a critical mass adoption to be effective. In this paper, we present WiFiTrace, a network-centric approach for contact tracing that relies on passive WiFi sensing with no client-side involvement. Our approach exploits WiFi network logs gathered by enterprise networks for performance and security monitoring, and utilizes them for reconstructing device trajectories for contact tracing. Our approach is specifically designed to enhance the efficacy of traditional methods, rather than to supplant them with new technology. We designed an efficient graph algorithm to scale our approach to large networks with tens of thousands of users. The graph-based approach outperforms an indexed PostgresSQL in memory by at least 4.5X without any index update overheads or blocking. We have implemented a full prototype of our system and deployed it on two large university campuses. We validated our approach and demonstrate its efficacy using case studies and detailed experiments using real-world WiFi datasets.

==> design_challenges.tex <==
\section{Deployment Challenges}
\label{sec:design_challenges}

\begin{enumerate}
    \item Privacy
    %\item Validation via User Study
    \item WiFi Dynamics/Ping-pong : The trajectories extracted from raw traces will be inherently noisy. For example, mobile devices may connect to access points that not the most proximal, or “ping-pong” between nearby access points even though the user is stationary. Similarly, when the user is walking to a new location, devices may connect to distant APs in weakly connected regions or exhibit similar ping-pong switching effects. Since we are using the AP location to determine the device location, all of these effects introduce noise or spurious location changes into our extracted trajectories. To address this issues, the raw traces are subjected to a multiple filtering and smoothing steps during trajectory extraction to remove noise and obtain clean trajectories for each device. Due to space constraints, full details of these smoothing and filtering steps for data cleaning may be found in [1] (anonymous TR is available upon request through the PC chair).
    
    \item Handling Multiple Devices
    \item Location Granularity
    \item Connection to distant APs when in open spaces eg. Field etc
    \item Walking outside buildings and getting connected to level 1 APs
    \item False positives but fewer false negatives
    \item Impact of aggressiveness of devices in drifting
\end{enumerate}

\subsection{Privacy Considerations:}
Since contact tracing technologies use location and proximity information of users, they raise important privacy concerns. Privacy concerns for client-side bluetooth-based applications are well known \cite{}. Since, network-centric client tracing is an alternative approach that raises a different set of concerns, we discuss these issues in this section and describe techniques used in out ongoing deployments to mitigate them.

First, our network-centric tool is aimed at health-care and medical professionals who perform contact tracing and not at end-users. Contact tracing is a decades-old approach that has traditionally been performed manually through questionnaires. Our tool has been designed to fit into this workflow and serves as an additional source of information for professionals engaged in contact tracing. Unlike some bluetooth-based apps, it does not allow end-users to lookup information about themselves or anonymous infected users. By focusing on health professionals and not end-users, our tool avoids some of the privacy pitfalls from giving end-users access to anonymous proximity data.

Second, even though data access is limited to health professionals the tool and its data us still prone to privacy misuse. there are two approaches for handling these problems. First, we strongly suggest that operational control of the tool be in the hands of the organization's IT security team. Recall that the approach is based on WiFi network monitoring data that is already routinely gathered by IT departments for network performance and security monitoring. For example, our campus uses such data to track down compromised devices that are inadvertently connected to our WiFi network and may be responsible for DDOS attacks from inside.

Since the IT department already has access to the raw data used by a network-centric tool deploying the tool does not increase privacy risks (since the same raw data is prone to the same privacy risk independent of our tool and IT departments have strict safeguards in place to protect such data by limiting access). Here, limiting operational control to the organization's IT provides good privacy protection.

However, it may not always be feasible to limit control of the tool to IT professionals alone. For instance, larger outbreaks of a disease may require allowing access to health officials who are performing contact tracing. In this case, we can address privacy concerns by not storing user identities or real MAC addresses with the tool instead. Instead, user names and device MAC addresses are anonymized by a cryptographic hash (eg SHA-1024). All queries on the tool are done using hashed identities and not real one. The full mapping of user names and device MAC addresses to their hashed values is stored separately and this information is accessible only to a small trusted group. To perform contact tracing on an individual this trusted person needs to authorize it (eg once consent is obtained) by releasing the mapping of actual name and MAC to the hashed values. The tool can then be queried using the hashed values. The tool can then be queried using the hashed value of that users information. Similarly once proximity reports are generated they can be sent to the trusted person, who can then deanonymize that information. In this manner, it is not possible to query the tool to track activities of an arbitrary user, unless first authorized, which prevents misuse. Our current campus deployment uses this anonymized data approach for additional safety.

Finally many countries have strict privacy laws that require user consent before using sensitive data. To comply organizations require users to consent to monitoring and gathering network data for critical safety operations - a prerequisite for such network monitoring. Further, health care professionals are required to obtain user consent to perform manual contact tracing a process that can be used for network centric contact tracing as well.

==> model.tex <==
\section{Model}
\label{sec:model}
\\
Model : [1 page]
\\
\subsection{Problem Formulation}
%: Mathematical Formulation

\subsection{Model Architecture}
\\
Architecture Diagram or
Model Pipeline diagram of LSTM based regression + battery scheduler module
\\
Para 1:
\\
LSTM based regression. 
\\
How it works.
\\
Some mathematical equations
\\
Para 2:
\\
Input and Output of the LSTM regressor
\\
Para 3:
\\
Battery scheduler algorithm
\\
Parameters considered for optimization

==> privacy.tex <==
\section{Privacy Considerations:}
\label{sec:privacy}

Since contact tracing technologies use location and proximity information of users, they raise important privacy concerns. Privacy concerns for client-side Bluetooth-based applications are well-known \cite{cho2020contact}. Since network-centric client tracing is an alternative approach that raises a different set of concerns, we discuss these issues in this section and describe techniques used in our ongoing deployments to mitigate them.

First, our network-centric tool is aimed at health-care and medical professionals who perform contact tracing and is not an end-user focused tool for self-monitoring prior contacts. Contact tracing is a well-established approach that has traditionally been performed manually through questionnaires \cite{eames2003contact}. Our tool has been designed to fit into this workflow and serves as an additional source of information, in addition to interviews, for professionals engaged in contact tracing. Unlike some Bluetooth-based apps, it does not allow end-users to lookup information about themselves or anonymous infected users. By focusing on health professionals and not end-users, our tool avoids some of the privacy pitfalls from giving end-users access to anonymous proximity data.

Second, even though data access is limited to health professionals, the data contains sensitive location information and is still prone to privacy misuse. There are two approaches to handling this problem. First, we recommend that operational control of the tool be in the hands of the organization's IT security group. Recall that the approach is based on WiFi network monitoring data that is already routinely gathered by IT departments for network performance and security monitoring. For example, our campus uses such data to track down compromised devices that are connected to our WiFi network and may be responsible for DDOS attacks from inside. Another example is tracking down student hackers, since the hacking of university computers (e.g., to change course grades) is a common exploit on university campuses. Audit and compliance laws in many regions also necessitate gathering network logs for subsequent analysis and audits. To address these issues, IT departments routinely collect detailed network logs and use them for optimizing performance or handling security incidents.

Since the IT department already has access to the raw data used by our network-centric tool, deploying the tool within the IT department does not increase privacy risks (since this raw data is already prone to the same privacy risks independent of our tool, and IT departments have strict safeguards in place to protect such data and limit access to it). Here, limiting operational control of the tool to the organization's IT group can provide good privacy protection in practice.

However, it may not always be feasible to limit control of the tool to IT professionals alone. For instance, larger outbreaks of disease may require allowing direct access to health officials who are performing contact tracing. In this case, we can address privacy concerns by not storing user identities or real MAC addresses with the tool itself. Instead, user names and device MAC addresses are anonymized by a cryptographic hash (eg SHA-2 hash). All queries on the tool are done using hashed identities and not the real ones. The actual mapping of user names and device MAC addresses to their hashed values is stored separately from the tool, and this information is accessible only to a small trusted group. To perform contact tracing on an individual, this trusted person needs to authorize it (e.g., once user consent is obtained) by releasing the mapping of the actual name of the user and their device MAC to the hashed values.  The tool can then be queried using the hashed values of that user's information. Similarly, once proximity reports are generated, they can be sent to the trusted person, who can then deanonymize that information using the mapping table. In this manner, it is not possible to query the tool to track activities of an arbitrary user, unless first authorized, which prevents misuse. Our current campus deployment uses this anonymized data approach for additional safety.

Finally, many countries have strict privacy laws that require user consent before collecting sensitive data. To comply, many organizations require users to consent to their IT policy that enables them to gather network data for critical safety operations---a prerequisite for such network monitoring. Further, health care professionals are required to obtain user consent to perform manual contact tracing---a process that can be used for network-centric contact tracing as well.\footnote{These professionals can decide whether to pro-actively notify co-located individuals who are deemed to be at risk during an outbreak or to publicize a list of locations and times visited by an infected individual(s) and request other users to contact them if they are impacted. In the latter case, the proximity report data is used for further contact tracing once co-located users contact health officials. The latter approach is presently used on our USA campus.}


